Exploring Defeasibility in Causal Reasoning

Defeasibility in causal reasoning implies that the causal relationship between cause and effect can be strengthened or weakened. Namely, the causal strength between cause and effect should increase or decrease with the incorporation of strengthening arguments (supporters) or weakening arguments (defeaters), respectively. However, existing works ignore defeasibility in causal reasoning and fail to evaluate existing causal strength metrics in defeasible settings. In this work, we present $\delta$-CAUSAL, the first benchmark dataset for studying defeasibility in causal reasoning. $\delta$-CAUSAL includes around 11K events spanning ten domains, featuring defeasible causality pairs, i.e., cause-effect pairs accompanied by supporters and defeaters. We further show current causal strength metrics fail to reflect the change of causal strength with the incorporation of supporters or defeaters in $\delta$-CAUSAL. To this end, we propose CESAR (Causal Embedding aSsociation with Attention Rating), a metric that measures causal strength based on token-level causal relationships. CESAR achieves a significant 69.7% relative improvement over existing metrics, increasing from 47.2% to 80.1% in capturing the causal strength change brought by supporters and defeaters. We further demonstrate even Large Language Models (LLMs) like GPT-3.5 still lag 4.5 and 10.7 points behind humans in generating supporters and defeaters, emphasizing the challenge posed by $\delta$-CAUSAL.

==> defeasible_reasoning/discussions.tex <==
\input{defeasible_reasoning/discussions/challenges}

\input{defeasible_reasoning/discussions/cesar}

==> defeasible_reasoning/research_questions.tex <==
We mainly conduct our experiments focusing on the following research questions: 
\begin{itemize}
    \item Research Question \RNum{1}: What is the existing pre-trained models’ ability in understanding temporality for causal reasoning? Specifically, we investigate whether language models can reason the cause based on both short-term information and long-term information. 
    \item Research Question \RNum{2}: Can language models generate correct defeaters for given causal facts that can make the causality less justified or more justified? Specifically, we explored whether existing language models generate assumptions or defeaters correctly. 
    \item Research Question \RNum{3}: How to precisely estimate on causal strength of causality? Specifically, can existing metrics on causal strength precisely estimate the intensity of causality and reflect the changes brought by supplementary information like assumptions or defeaters? We answer Research Question \RNum{1} and Research Question \RNum{2} in \S \ref{sec:experiment:rq1} and \S \ref{sec:experiment:rq2} respectively. We thoroughly investigate Research Question \RNum{3} in \S \ref{sec:discussions}. 
\end{itemize}

